Post-hoc Uncertainty Learning using a Dirichlet Meta-Model

It is known that neural networks have the problem of being over-confident when directly using the output label distribution to generate uncertainty measures. Existing methods mainly resolve this issue by retraining the entire model to impose the uncertainty quantification capability so that the learned model can achieve desired performance in accuracy and uncertainty prediction simultaneously. However, training the model from scratch is computationally expensive and may not be feasible in many situations. In this work, we consider a more practical post-hoc uncertainty learning setting, where a well-trained base model is given, and we focus on the uncertainty quantification task at the second stage of training. We propose a novel Bayesian meta-model to augment pre-trained models with better uncertainty quantification abilities, which is effective and computationally efficient. Our proposed method requires no additional training data and is flexible enough to quantify different uncertainties and easily adapt to different application settings, including out-of-domain data detection, misclassification detection, and trustworthy transfer learning. We demonstrate our proposed meta-model approach's flexibility and superior empirical performance on these applications over multiple representative image classification benchmarks.

==> sections/application.tex <==
\section{Uncertainty Quantification Applications}
In this section, we will discuss several important applications that can be tackled using our proposed post-hoc uncertainty learning framework. 
%Given the pretrained model $\vh$ and its training data $\mathcal{D}_{B}=\left\{\boldsymbol{x}^B_{i}, y^B_{i}\right\}_{i=1}^{N_B}$, the goal is to efficiently train the meta-model $\vg$ using the exiting training data. 
Our meta-model has two major advantages: (1) It is efficient, i.e., it is easy to optimize and empirically require less number of training data due to smaller model complexity, (2) It is versatile, i.e., it not only can quantify different uncertainties to adapt to different applications, but also different settings, i.e., like transfer learning, the distribution of training data for meta-model can even be different from the base-model.
\paragraph{Out of domain data detection}
The base-model $\vh$ is trained using data sampled from distribution $P^B_{Z}$. During testing, if there exists some unobserved out of domain data from another distribution $P^{ood}_{Z}$, the meta-model should correctly identify the in-distribution or out-of-distribution input sample. We use the same training set as base model to train the meta-model, i.e., $\mathcal{D}_{B} = \mathcal{D}_{M}$, which means our proposed method does not require additional OOD data for training. For OOD task, we use three epistemic uncertainties to measure the uncertainty score $\vu\left(\tilde{y}\right)$.
\paragraph{Miss-classification Detection}
Instead of detecting whether a testing sample is out of domain, the meta-model aims to identify the failure or success of prediction during testing. We train the meta-model with the same setting as OOD detection task, and use the two total uncertainties.
\paragraph{Trustworthy Transfer Learning}
The aforementioned applications assume the data used for training the base-model and the meta-model are exactly same, i.e., $\mathcal{D}_{B} = \mathcal{D}_{M}$, or $P^B_{Z} = P^B_{M}$ in general. Instead, the transfer learning assumes there exists a pretrained model $\vh_s$ trained using source task data $\mathcal{D}_{s}$ sampled from source distribution $P^s_{Z}$, and the goal is to adapt the source model to target task using target data $\mathcal{D}_{t}$ sampled from target distribution $P^t_{Z}$. Most existing transfer learning problem focus on improving the prediction performance of transferred model, but ignore its uncertainty quantification performance on the target task. Our meta-model method can be utilized as a simple and effective way to address this problem, i.e, given pretrained source model $\vh \circ \vf = \argmin_{\vh \circ \vf} \gL_E(\vh \circ \vf,\gD_s)$, the meta-model can be efficiently trained using target domain data, i.e., $\vg = \argmin_{\vg} \gL_E(\vg \circ \vf,\gD_t)$.  

==> sections/rebuttal.tex <==
\section{Rebuttal}
We thank the reviewers for their detailed feedback and valuable suggestions to help us further improve this work. We address their concerns through this response and will include more detailed results in the final version.

\subsection{Response to Review-1:}

\paragraph{(1) Results of Calibration:}
Our method has demonstrated strong performance on the selective classification, which is directly related to model calibration and requires an accurate estimation of the total uncertainty. As per the reviewer's suggestion, we computed the ECE scores of our methods and other baseline methods. 
CIFAR10: Ours(10.4), Base-Model(13.2), LULA(10.8), BeBayesian(10.6), MCDropout(11.3); 
CIFAR100: Ours(7.3), Base-Model(26.2), LULA(7.1), BeBayesian(5.8), MCDropout(22.5). 
It shows that our method achieves comparable or better calibration performance than the baseline methods.

\paragraph{(2) Comparison with existing meta-modeling approach:}
To the best of the authors' understanding, Chen et al. 2019 and Jain et al. 2021 are the only existing meta-model-based UQ works. It’s possible that we misunderstood the reviewer’s request, but we already compared with Chen et al. 2019 (denoted as "Whitebox") in the experiment section and demonstrated that our method outperformed it across different tasks. Additionally, we note that Jain et al. 2021 mainly focuses on regression instead of classification and should be considered contemporaneous. We leave comparison with this work for future work.
%, its problem setting mainly focuses on regression instead classification
%, and it is still unpublished. Thus, a direct comparison may not serve the purpose at this time.

\subsection{Response to Review-2:}

\paragraph{(1)}
Thanks to the reviewer for pointing out the typo in Table 1. We will correct it in the revision.

% , and we are sure that our experiment setups are all accurate

\paragraph{(2) Difference between our work and prior network:}

First, the motivations and problem settings are different. Our work tries to improve the uncertainty quantification performance of an arbitrary pre-trained model in a post-hoc manner. Prior Network [1] aims to train a Bayesian model with the UQ capability from scratch. Second, the Dirichlet technique used in this work, though it might be similar to [1], simply serves as one efficient technique to quantify epistemic uncertainty. However, our method is not limited to using the Dirichlet technique as long as the output of the meta-model can quantify total and epistemic uncertainties. Moreover, compared to [1], our proposed method uses the variational loss instead of the KL divergence loss that requires additional OOD data defined by Equation 12 in [1]. In the revision, we will further clarify the main differences.

\subsection{Response to Review-5:}

\paragraph{(1) Comparison with existing OOD work ALOE[1]:}

The relation between UQ and OOD has been discussed in section 5.1, and we agree that we can introduce more about OOD in the related work. The scope of this work is to propose a general approach that can quantify different types of uncertainties for various tasks, especially in a challenging post-hoc setting. The OOD detection task considered here is a specific application that highly relies on good epistemic uncertainty. However, the existing OOD detection approach is not necessarily capable of the general UQ capability for other applications, such as selective classification that relies on total uncertainty. 


As the reviewer suggested, we compare with [1] to further validate our method.  The results are the AUROC scores evaluated on CIFAR 10 and CIFAR 100 (average over five OOD datasets). CIFAR10: Ours-MI(98.4), ALOE(97.3);  CIFAR100: Ours-MI(87.4), ALOE(86.9). Our method can still demonstrate advantages over ALOE on OOD tasks. Moreover, ALOE [1] requires an additional OOD dataset for training their model, while our method does not. Besides, we notice that training ALOE is computationally expensive. %that takes half day.
We will cite [1] in the final version and provide more discussion and comparison. 

\paragraph{(2) Comparison with Calibration approach [2]:}

Traditional calibration approaches, such as temperature scaling [2], have two major limitations. First, it requires an additional validation dataset to optimize the temperature. Second, as we mentioned in the third paragraph of the introduction section, calibration methods fail to capture epistemic uncertainty, which is crucial for OOD detection. To further elaborate this argument, we evaluate the performance of the calibration approach [2] on OOD detection and provide the average AUROC score: CIFAR10: Ours-MI(98.4), Base-Model(87.9), Calibration[2](92.3); CIFAR100: Ours-MI(87.4), Base-Model(75.8), Calibration[2](82.5). The calibration can improve the performance over the base model, but our proposed method can still outperform calibration [2] by a large margin.


\subsection{Response to Review-6:}

\paragraph{(1) Demonstrate the efficiency:}

Our meta-model-based approach is much more efficient than traditional uncertainty quantification approaches because it has a simpler structure and faster convergence speed. To quantitatively demonstrate such efficiency, we measure the wall-clock time of training the meta-model in seconds (on a single Titan RTX GPU): CIFAR10/VGG16: 66.5s (for five epochs); CIFAR100/WideResNet: 241.9s (for ten epochs). The training time of the meta-model can be negligible compared to those approaches training the entire base model from scratch (usually taking several hours).








%As the reviewer suggested, we compare with [1] to further validate our method.  The results are the AUROC scores evaluated on CIFAR 10 and CIFAR 100 (average over five OOD datasets). CIFAR10: Ours-MI 98.4(100.0, 98.8, 95.2, 98.1, 100.0), ALOE 97.3(99.9, 98.3, 92.1, 99.9, 96.2); CIFAR100: Ours-MI 87.4(94.3, 84.4, 81.9, 85.5, 90.8), ALOE 86.9(99.9, 86.9, 70.2, 85.3, 92.2). Our method can still demonstrate advantages over ALOE on OOD tasks. Moreover, ALOE [1] requires an additional OOD dataset for training their model, while our method does not. Besides, we notice that training ALOE is computationally heavy that takes half day. We will cite [1] in the final version and provide more discussion and comparison. 
